Streetify: Using Street View Imagery And Deep Learning For Urban Streets Development

The classification of streets on road networks has been focused on the vehicular transportational features of streets such as arterials, major roads, minor roads and so forth based on their transportational use. City authorities on the other hand have been shifting to more urban inclusive planning of streets, encompassing the side use of a street combined with the transportational features of a street. In such classification schemes, streets are labeled for example as commercial throughway, residential neighborhood, park etc. This modern approach to urban planning has been adopted by major cities such as the city of San Francisco, the states of Florida and Pennsylvania among many others. Currently, the process of labeling streets according to their contexts is manual and hence is tedious and time consuming. In this paper, we propose an approach to collect and label imagery data then deploy advancements in computer vision towards modern urban planning. We collect and label street imagery then train deep convolutional neural networks (CNN) to perform the classification of street context. We show that CNN models can perform well achieving accuracies in the 81% to 87%, we then visualize samples from the embedding space of streets using the t-SNE method and apply class activation mapping methods to interpret the features in street imagery contributing to output classification from a model.

==> Streetify Arxiv/conclusion.tex <==
%\section{Conclusion}

%This paper has investigated the use of convolutional neural networks for analyzing urban streets through street view imagery at the scale of entire cities. Given the current relative dearth of label street view imagery in the machine learning community, our models can  label street view imagery of Boston and San Francisco with accuracy of at least 81\% to 87\%. This was possible with limitations on the amounts of data provided free of cost through the Google API which was challenging. Given a subset of the streets in a city, the model can automatically and much faster perform the classification of all the streets in a city once it learns from a considerably enough subset of labeled streets. We hope that it can help other researchers in machine learning, smart cities, urban planning, and related fields in their work on understanding cities. We set out to study patterns of street contexts, as being able to quantify such patterns will enable richer applications in topics such as urban design and planning, infrastructure benchmarking, transportation engineering and socio-economic composition of communities. We formulated this as a two-step task: first predicting street context classes from street view imagery, then turning this (rigid) classification into a continuous spectrum by embedding the features extracted from the convolutional classifier into a lower-dimensional manifold. We show that the classification task achieves encouraging results, given the large variety in physical appearance of urban settings having the same functional class. Moreover, we exemplify how the features extracted from the convolutional network allow for identifying "neighbors" of any given query image, allowing a rich comparison analysis of street contexts by their visual composition. The analysis in this paper shows that some types streets contexts are easier to infer than others. For example, in all our experiments, the models had most trouble predicting the Residential Throughways due to the many shared visual attributes it has with other classes. However, Park streets tend to be visually similar across the city and usually very dominated by greenery on both sides. We then investigate some of the visual features responsible for the activation of certain class predictions. For parks for example, the CAM method produced heatmaps with heat heavily centered around trees and vegetation. The CAM results helped us validate the visual features that are activating our models to predict a certain class. We include more samples from the CAM results on the \texttt{github} page of the project.

%A future direction of this work is exploring the extent to which the models are extendable and transferable to other cities. As such, for several classes we can expect learning to transfer from one geography to another. Thus, while it is not news that some cities are more "similar" than others (Boston is more similar to Providence than San Francisco), the methodology in this paper allows for a more quantitative and practical comparison of similarity. By leveraging street view imagery (available virtually world-wide), this approach may allow for a low-cost way to classify streets in locations where ground truth information on street contexts is not available.  In addition and as future directions of this work, we plan to i) continue to develop more rigorous ways to compare and benchmark urban streets, going deeper to physical elements (stores, sidewalks, street signs etc.); ii) improve and further curate models that can generate open urban street datasets; and iii) extend this type of analysis to more cities across other geographical locations.

%\section{Practical Training Details}
%We used ADAM optimization for the loss function (a standard multi-class cross-entropy). For the CNN architectures of ResNet and AlexNet, we used a learning rate of $5\times10^{-6}$. For the Inception model we used a learning rate of $1\times10^{-4}$. We used a batch size of 50 and trained for 2000 epochs for each of the architectures or until the validation error remains the same for more than 20 epochs. The trained models are available on the \texttt{github} page mentioned earlier of the project as the well as the codes used to develop the model and prepare the data. In all our experiments, we used popular data augmentation techniques, including random horizontal flipping of the input images, random rotation (up to 40 degrees). Input images were 200$\times$100$\times$3 pixels in size (RGB bands), each image is composed of 100$\times$100$\times$3 left view and another one for right view concatenated as an input to the model. We implemented the models using open-source deep learning framework \texttt{Pytorch}. We use an Nvidia RTX2080ti GPU card to training CNN models. To handle the issue of the imbalance in the classes of streets contexts, we sample training images with weights. The lower the amount of images from a class the higher their sampling weight and vice versa. We then can sample equivalent number of images from each class for the training and testing phases. We used the t-SNE implementation of the \texttt{scikit-learn} python library to visualize the feature vectors. We used the euclidean distance as a metric to calculate the distances. We ran it to project the feature vectors on a space of dimension 2 and with perplexity 2.




==> Streetify Arxiv/data.tex <==
\section{Data}
The city of San Francisco developed a manual process by which street contexts are determined. In this section, we first discuss the manual process of street context classification in urban planning developed by the city of San Francisco \cite{SF_BSP}. Then, we proceed by discussing how we sample labeled street imagery data for the purpose of training a deep convolutional neural network to perform the task of street context classification.
\begin{figure}[!ht]
	\begin{center}
		\includegraphics[width=\linewidth]{plots/SF_classes_larger_label-min.png}
		\caption{The road network of San Francisco with labeled street contexts.}
		\label{fig:SF_labels}
	\end{center}
\end{figure}

\subsection{The manual street context classification process}
The city of San Francisco developed a manual process by which street contexts are determined\cite{SF_BSP}. The inputs of this manual process of street context classification are the shapefiles of the unlabeled streets in a city and the use of parcels on the sides of the streets (i.e. commercial, residential...etc). We first collect the streets shapefile for the city of interest, the data is usually made available by city councils. The shapefile data for the streets of Boston and San Francisco were graciously provided by the city councils (San Francisco streets were already labeled by the city council). The city also shared the manual process used by their urban planners to perform the classifications of street contexts. We then followed the manual process to label streets in Boston. The labeling scheme results in 11 classes for the city of San Francisco and 10 classes for the city of Boston. This is due to the reason that there is little to no presence of the \textit{Downtown Residential} class in the downtown of Boston. 
  \begin{figure}[!h]
 	\begin{center}
 		\includegraphics[width=\linewidth]{plots/sample.pdf}
 		\caption{ (From the left) Commercial Throughway, Downtown Commercial and Alley in Boston.}
 		\label{fig:threeSamples}
 	\end{center}
 \end{figure}


The streets are labeled based on conditions pertaining to transportational functionality and the use of land on the sides. The San Francisco classification scheme developed by the city's urban planners is a multistage scheme for classification of streets that can be summarized in the following steps: 
\begin{enumerate}
\item Determine the side use context: Streets are distinguished by their side use using parcel information including side contexts of \textit{commercial} and \textit{residential}. 
\item Determine the transportation context: we then assigning labels that pertain to transportational features of the street. This includes  \textit{throughway}, \textit{highway} and \textit{highway ramps}. Streets with lower flows are labeled \textit{dowtown} and \textit{neighborhood} for their transportation context. 
\item Identify special conditions: certain streets have special classifications including \textit{alleys}, \textit{parks}, \textit{industrial}.  
\end{enumerate}
\subsection{Sampling labeled street imagery:}
   Figure \ref{fig:SF_labels} shows the 11 classes for the city of San Francisco. Streets of the class \textit{Neighborhood Residential} constitute the majority of the streets. The process of classification for the city of SF was conducted by the city council. We followed the same process to label subset of streets in Boston for this study.

%\textbf{Street classes in further detail:}
 %There are two Downtown street contexts, the \textit{Downtown Commercial} and \textit{Downtown Residential} are streets that are in the downtown area and have businesses or living spaces accordingly. Then there are \textit{Neighborhood Commercial} and \textit{Neighborhood Residential} which have lower car flow and are usually further away from the center of the city and have business and apartments/houses on their sides respectively. Then there are Throughways, \textit{Commercial Throughway} and \textit{Residential Throughway}. Those are usually wider streets and have higher speed limits, thus allowing for more car flow. Then there are the \textit{Highway} and \textit{Highway ramp} classes. The Highway includes interstates and the ramps are the connectors for entries and exits to highways. The classification also has a set of special classes for \textit{Alley}, \textit{Park} and \textit{Industrial}. \textit{Alleys} are very narrow streets that are in the back side of buildings for services access. \textit{Park} are streets that pass through parks in the city. \textit{Industrial} are in places of factories and logistical activities.

Once a set of streets in a city is labeled according to the manual process of street context classification discussed in the previous subsection, we then can use the shapefiles of streets to sample labeled street view imagery. First, we randomly sample a street segment from the subset of labeled street segments without replacement. Then, we sample a random lat/lon from the sampled street segment. We then proceed to collect images that capture  sides of the street as well as the road ahead.  Images provided by the Google Street View API cover an angle of approximately 90 degrees.  To cover the sides of the street while maintaining view on the road, we collect two Images one tilted towards the right of the direction of traffic on the street and the other tilted towards the left of the direction of traffic on the street. The pair of images that we sample are labeled with the street context label as per the shapefile. %Figure \ref{fig:Sample Classes Images} shows sample labeled images taken in Boston.

 The Google Street View images API \cite{streetViewApi} provides street view imagery as a service. The service provides a free quota for the use of the API that we utilize for the purpose of this study, the free quota is renewed every month. The API takes the lat/lon of a location as well as an angle of view and returns images of varying sizes and maximum size of 640x640 pixels. Figure \ref{fig:threeSamples} shows sample points on the street road network and the corresponding views from the street view API. In orange frame are the images taken with an angle towards the left and in blue frame are images that are taken towards the right of the direction of the street. From left to right of the figure we have a Commercial Throughway, a Downtown Commercial and an Alley from Boston. Each sample image has a map below it showing the location where the lat/lon and view angle of the images.

%\begin{figure}[!h]
%	\advance\leftskip-4cm
%	\begin{center}
%		\includegraphics[width=\linewidth]{plots/sample1.png}
%		\caption{Boston street contexts sample}
%		\label{fig:Sample Classes Images}
%	\end{center}
%\end{figure}
 %In figure \ref{fig:Sample Classes Images} we show a sample images for every street context class in the city of Boston. There are 10 major street context classes in the city of Boston. Similar to San Francisco, the majority of classes of the streets are the \textit{Neighborhood Residential}.

% In Table \ref{tab:stats} we present summaries of the training dataset that we use for models training in this paper. This dataset consists of images in Boston and San Francisco. The amounts of labeled imagery data we used to train the model was limited by the free quota allowed through the Google Street View API\cite{streetViewApi}. We collect around 29k images for the both cities in total, around 15k images for each city. The data is split into 80\% for training and 20\% for validation.  The model would benefit from having more data for better generalization. We try to sample balanced set of images per class, however some classes are much more abundant than others in a city due to their respective urban nature. In Boston for example, the number of \textit{Alley} streets is less frequent to observe compared to other classes. On the other hand, there is an abundance of Neighborhood Residential streets in the city compared to other classes.
 %\begin{table}[!b]
 %	\begin{tabular}{|l|c|c|c|c|}
 %		\hline
% 		class/city             & Boston & San Francisco   \\ \hline
% 		Alley                  &  700    &   1252           \\ \hline
% 		Commercial Throughway  &   1462     & 1336    \\ \hline
% 		Residential Throughway  &  1368    & 1272                 \\ \hline
% 		Downtown Commercial    &   1748     & 1197                 \\ \hline
% 		Downtown Residential   &     -   & 922                 \\ \hline
% 		Highway				   &  2012      & 1202                \\ \hline
% 		Highway Ramp		   &   1476     & 1002                 \\ \hline
% 		Industrial			   &    1060    & 1328                \\ \hline		
%         Park			   &    1044    & 1580                \\ \hline		
% 		Neighborhood Commercial&    1036    & 1242                 \\ \hline
% 		Neighborhood Residential&   2818     & 1434                \\ \hline
% 	\end{tabular}
% 	\captionof{table}{The counts of images for the sampled points in the different cities in the study.} \label{tab:stats}
% \end{table}

%The imbalanced nature of street classes in the cities of Boston and San Francisco shows in the set of data we collected for purposes of training and validation. Table \ref{tab:stats} shows that there aren't many alleys in Boston or \textit{Downtown Residential} streets in San Francisco. The table also shows that there is an abundance of Neighborhood Residential contexts in both Boston and San Francisco. We address the issue of the class imbalance for purposes of training a model later in this paper.
%some statistics of the data to be used in the model


==> Streetify Arxiv/intro.tex <==
\section{Introduction}
%\begin{itemize}
%\item here goes the motivation of the problem. Answer the following question:
%\item what is the problem, where does it come from?
%\item why is this problem important, namely why do we need street context classification? 
%\item where can this be used and for what purposes?
%\item its possible to link the work to self driving cars. one way is to say that self driving cars can benefit from knowing the context of streets? They should be more cautious to pedestrians when traveling in commercial areas and parks.
%\end{itemize}

%Cities today are growing very rapidly and are expected to be home for around 70 percent of world's population by 2050\cite{rode2011cities}. With the rapid urban population growth, cities' infrastructures are becoming data generation engines while needing to coop with the rapid growth in population. To coop with rapid growth of cities, urban planners are continuously innovating and revisiting methods and techniques of planning and design. With the rapid ubiquity of the internet and communication technologies, the internet is increasingly becoming home to large datasets pertaining to cities. In this paper, we explore one way to take advantage of the availability of city street view imagery to help city authorities and planners with street classification faster and at larger scales in an automatic fashion.

%the existing classification methods and the SF prpoposed method
Cities today are growing very rapidly and are expected to be home for around 70 percent of world's population by 2050\cite{rode2011cities}. Transportation engineers and urban planners traditionally classified streets on the road network in cities based on vehicular transportational features. Such street classifications include arterials, major roads, minor roads, connectors and so forth. Although such classification is very useful in terms of vehicular transportation planning, it doesn't differentiate between streets that pass through residential versus commercial areas for example, where the differentiation is of at most importance to design and build more livable and sustainable streets. Recently, a significant emphasis to increase focus on the \textit{context} of a street in the process of urban planning have become very noticeable. The \textit{context} of a street encompasses the use of land on the sides of a street in addition to its vehicular transportational characteristics. 

Several city and state authorities have started proposing extensions for the traditional classification of roads towards one that encompass the use of the sides of the streets.  For example, chapter 4 of the guidebook for transportation planning from the state of Pennselvania elaborates on the supremacy of \textit{street context} over traditional transportation classification methods for purposes of developing more livable and sustainable cities\cite{guidebook2008planning}.  The state of Florida Department of Transportation (FDOT) started adopting new classification methods of \textit{street context} that goes beyond the traditional classifications of streets\cite{FDOT_ContextClassification}.  The city of San Francisco adopted an extended street classification scheme to govern how the city designs, builds, and maintains its pedestrian environment, the classification scheme is called the Better Street Plan (BSP). The intent for it is to become the corner stone for developing streets that are more livable\cite{SF_BSP}. In this paper, we illustrate a way to automate the process of BSP classification of streets in San Francisco and Boston using computer vision and street view imagery. 

%Computer vision is one of the prominent areas of machine learning and AI, it employs approaches and techniques from machine learning for computers to develop models with high level understanding of images and videos data. The recent developments in the area of deep learning have been very successful in tasks such as image classification, object recognition and detection. The scientific domain of applications hasn't been of a particular focus for researchers developing the method most of the time. This provides room for researchers to contribute in applying computer vision to application domains. 

%The following section starts with an exploration of the potentials of using deep learning with street view images to develop a tool that can aid in the process of city planning.

 978-1-7281-0858-2/19/$31.00 © 2019 IEEE 
 
With the ubiquity of technology today, we have access to data on massive scales that can alleviate challenges of urban data collection and tedious data entry\cite{zheng2014urban}. There has been applications in domains of urban sciences, transportation and socio-economic sciences\cite{lazer2009life,alhasoun2017city,zhang2018social}. Its is also at the core of the relatively new field of urban computing\cite{zheng2014urban}. An example of data that became available with the ubiquity of technology in cities is street imagery data. The dataset is usually collected by moving cars with cameras. The data is then aggregated and used for the public to browse and view different places. Example efforts of such data collection include the Google Street View\cite{streetViewApi}. Another example of effort of crowd sourcing the collection of street view imagery includes Mapilary which proved successful at collecting considerably large amounts of street imagery data worldwide\cite{mapilary}. We aim to show that this dataset can be used with models of computer vision to aid urban development.

We summarize our contributions in the following points:
\begin{itemize}
\item We develop the framework for building automatic \textit{street context} classification. The framework is composed of labeling and sampling street view imagery. Then training and validation of deep convolutional neural network models.
\item We test the framework on data gathered from the wild. Namely the cities of San Francisco and Boston where we have labeled \textit{street contexts}.
\item We illustrate the potential of such applications by reporting on CNNs achieving accuracies in the 81\% to 87\% range. 

\item  We then validate our models using t-SNE to visualize the streets embedding space. We apply Class Activation Mapping (CAM) methods for interpretability of the predicted classes\footnote{https://github.com/fha/streetContext}.
\end{itemize}






==> Streetify Arxiv/literature.tex <==
\section{Literature}
%there are applications of computer vision to the domain of urban sciences

There have been several interesting application of machine learning and particularly deep learning on imagery data in the domain of urban computing and remote sensing. Researchers from the domain of remote sensing have been focusing on developing models of inferring land use and land cover from satellite imagery\cite{albert2017using,Buslaev_2018_CVPR_Workshops,Zhou_2018_CVPR_Workshops,Hamaguchi_2018_CVPR_Workshops,Aich_2018_CVPR_Workshops,albert2017modeling}. Recently, researchers organized the Deepglobe challenge as part of the CVPR conference, the challenge focused on common challenges in remote sensing including road extraction, building detection and land cover classification \cite{demir2018deepglobe}. Researchers produced a myriad of approaches and deep learning techniques to address the challenging tasks\cite{demir2018deepglobe,zhou2018d,hamaguchi2018building,sun2018stacked,kuo2018deep}. Furthermore, researchers used street view imagery in congruence with satellite imagery to enhance the process of digitizing maps.  Cao et al. used an integrative approach of using satellite imagery and street view to infer land use then classify buildings and points of interest (POIs)\cite{cao2018integrating}.

%In this paper we make use of street view imagery to perform the task of classification of street context instead of satellite imagery. The resolution of freely available satellite imagery is not very high to the point that it doesn't provide sufficient visual features for street classification. Furthermore, for certain parts of the urban setting, high rise buildings obstruct the view of surrounding streets and the sides of the streets. Obstructions in the field of view of satellite imagery also occur in tunnels and streets under larger trees. In addition, stores and businesses are often not visible through satellite imagery, the top views of buildings are similar in many of the commercial and residential buildings. Satellite imagery would in many cases lack the information to distinguish between commercial and residential buildings on the sides of a street. For example in Boston, Marlbough and Newbury streets share very similar views through satellite imagery. However, Marlbourough street is considered residential and Newbury street is a common touristic attraction street of many shops, restaurants and cafes. 

Using street view imagery researchers showed how it can be a predictor to several urban socio-economic measures in cities. Gebru et al. developed an object detection model to extract cars from street view images, the paper then proceed by doing an image classification of the make, model and age of cars seen in a neighborhood area\cite{gebru2017using}. Then a lookup for the prices of the cars seen in images is performed against a database of their expected prices. The paper shows statistically significant correlations between demographics and the prices of cars residing in an area. They tested the strength of correlation of the metric of extracted car prices against several demographical features of urban areas, namely the U.S. Census and presidential voting data. Naik et al. used street view imagery to develop models that can predict the perceived safety of a street. They trained models against perceived street safety collected through surveying 7000 participant to input their perceived safety score given a street view image\cite{naik2014streetscore}. Naik et al. extended the work and developed a computer vision model to measure changes in the physical appearances of neighborhoods from street-level imagery across time. They studied the correlation of the magnitude of change to neighborhood demographical characteristics. They identified metrics that can predict neighborhood physical change, they found that education level and population density are strong predictors in magnitude of urban physical change of an area\cite{naik2017computer}. Kidzinski et al. used street view imagery of houses and apartment complexes to train a model against car insurance data. The paper shows predictive strength in visual features of houses towards predicting risk of car accidents. Given the address of insurance beneficiary, the model inputs street imagery of their home address and can outputs prediction of car accidents risk of an individual\cite{kita2019google}. The visual features in street view images are very rich enabling many applications of urban computing. We explore its potentials for urban planning towards better classifying streets in a city.










==> Streetify Arxiv/model.tex <==
\section{Modeling}
In this section we discuss the conceptual framework of the process and the architectures of the deep Convolutional Neural Networks (CNN) in our framework.
\subsection{The general framework}

Street context classification incorporates the side use of streets and land use of its sides in addition to the transportational attributes of a street. Side use of streets is influenced by the cultural and socio-economic functions the street servers (which is a subjective judgment by experts). Figure \ref{fig:25}-a illustrates the framework of street context classification of a city. The framework sampling street view imagery from labeled streets shapefile. The CNN model is trained to perform the classification. The CNN outputs a feature map in the embedding space of street contexts.  
 \begin{figure}[!h]
	\advance\leftskip-4cm
	\begin{center}
		\includegraphics[width=\linewidth]{plots/modelPipeline.png}
		\caption{The general framework architecture (a) The pipeline of labeling and sampling street view images then training a CNN model. (b) The continuous embedding space of street contexts.
}
		\label{fig:25}
	\end{center}
\end{figure}

We take the view that street context classes are just a useful discretization of a more continuous spectrum of patterns in the organization of fabric of streets in an urban setting. This viewpoint is illustrated in Figure \ref{fig:25}-b while some attributes (e.g., amount of built structures or vegetation) are directly interpretable, some others may not be. Nevertheless, these patterns influence, and are influenced by, socio-economic factors (e.g., economic activity), and dynamic human behavior (e.g. mobility, parking occupancy). We see the work on cheaply curating a large-scale street view classification dataset and comparing streets using deep representations that this paper puts forth as a necessary first step towards a granular understanding of urban settings in data-poor regions.

\subsection{Convolutional Neural Network (CNN) architectures}
%In 2012, Krizhevsky et al. applied a CNN to the Imagenet \cite{krizhevsky2012imagenet}. It was the first time an architecture was more successful than traditional, hand-crafted feature learning on the ImageNet. The AlexNet laid the foundations for the traditional CNN, a convolutional layer followed by an activation function followed by a max pooling operation. Much of the success of deep neural networks has been accredited to these additional layers. The intuition behind their function is that these layers progressively learn more complex features. The first layer learns edges, the second layer learns shapes, the third layer learns objects, and so on. In this section, we briefly describe the different architectures used in this paper for our purpose of street context classification. We start with the AlexNet then move to more recent ones including ResNet and Inception.

In 2012, Krizhevsky et al. applied a CNN to the Imagenet \cite{krizhevsky2012imagenet}. It was the first time an architecture was more successful than traditional, hand-crafted feature learning on the ImageNet. The AlexNet laid the foundations for the traditional CNN, a convolutional layer followed by an activation function followed by a max pooling operation. Much of the success of deep neural networks has been accredited to these additional layers. The intuition behind their function is that these layers progressively learn more complex features. The first layer learns edges, the second layer learns shapes, the third layer learns objects, and so on. In this paper, we explore various CNN architectures starting with the AlexNet then moving to more recent ones including ResNet and Inception \cite{krizhevsky2012imagenet,szegedy2016rethinking,he2016deep}.


 %Altough popular belief back then deeper models are to be expected to perform better,  He et al. \cite{he2016deep} empirically show that there is a maximum threshold for depth with the traditional CNN model. He et al. showed that the failure of deeper models would might be attributed to overfitting. However, they also showed that shorter models had lower error rates defying the overfitting argument.

%He et al. \cite{he2016deep} plot the training and test error of a 20-layer CNN versus a 56-layer CNN. This plot defies our belief that adding more layers would create a more complex function, thus the failure would be attributed to overfitting. If this was the case, additional regularization parameters and algorithms such as dropout or L2-norms would be a successful approach for fixing these networks. However, the plot shows that the training error of the 56-layer network is higher than the 20-layer network highlighting a different phenomenon explaining it’s failure.

%Evidence shows that the best ImageNet models using convolutional and fully-connected layers typically contain between 16 and 30 layers.


%\textbf{AlexNet Architecture:} 
%AlexNet was developed and trained on the ImageNet dataset where it performed very well in 2012\cite{krizhevsky2012imagenet}. It is a CNN named AlexNet, it contains 8 neural network layers, 5 convolutional layers and 3 fully-connected layers. Relu is applied after every convolutional and fully connected layer. Dropout is applied before the first and the second fully connected year. The AlexNet started the use of Relu activation instead of Tanh to add non-linearity. It accelerates the speed of training while maintaining similar accuracy. The model makes use of dropout instead of regularization to deal with overfitting. The network has around 60 million parameters, and needs around a billion computation units in a forward pass. 

%\textbf{ResNet architecture:} 
%The ResNet architecture has achieved state-of-the-art performance on image classification on several popular natural image benchmark datasets\cite{he2016deep}\cite{he2016identity}. It consists of blocks of convolutional layers, each of which is followed by a ReLU non-linearity. Each block in the convolutional base is followed by a max-pooling operation. Finally, the output of the last convolutional layer serves as input feature map for a fully-connected layer with a sofmax activation function. The key difference in this architecture is the implementation of shortcut connections that skip blocks of convolutional layers, allowing the network to learn residual mappings between layer input and output. The model is structured in a way to learn residues by passing the input to the output through a shortcut\cite{he2016deep}. This approach allows the model to grow its depth without having vanishing gradient issues. The ResNet models tested in this paper are the ResNet18, ResNet34 and ResNet50. 


%\textbf{Inception Architecture:}
%The Inception-v3 architecture is a convolutional neural network (CNN) which is 27 layers deep including the maxpooling layers. The main component in this network is the inception module, it is a combination of three convolutional layers of different kernel sizes: a $1\times1$ Convolutional layer, $3\times3$ Convolutional layer and $5\times5$ Convolutional layer with their output concatenated into a single output forming the input to the next layer. The Inception module allows the internal layers to pick and choose which filter size will be relevant to learn the required information, this is due to the different kernel sizes of the inception module. This allows for recognition of the same features in varying sizes between images\cite{szegedy2016rethinking}. 




==> Streetify Arxiv/results.tex <==
\section{Results and Validation}
In this section, we show the accuracies of the models per city, per model architecture. We show the confusion matrices of the Inception-v3 model on the validation set of Boston and San Francisco. The data was split 80\% for training/testing and 20\% for validation. 

%\begin{itemize}
%	\item make sure to include the following:
%	\item loss of training vs testing for the various methods of Resenet VGnet...etc
%	\item the confusion matrix of the selected model
%	\item the different accuracies of each model
%	\item take a sample street and show the images on it as well as the classification of the model versus the ground truth
%	\item how would you go about using the model to classify street segments.
%\end{itemize}
\subsection{Accuracy}
 Table I shows the accuracies of the different architectures trained on labeled images from the city of Boston and San Francisco. The AlexNet architecture achieves the lowest accuracy on the validation set for both cities. The Inception-v3 model achieves the highest accuracy on our validation set of both cities. For Boston, AlexNet has an accuracy of 83.16\% and Inception-v3 has an accuracy of 87.79\%. For San Francisco, AlexNet has an accuracy of 81.69\% and Inception-v3 has accuracy of 84.17\%. We notice a drop in accuracy between Boston and San Francisco for the same model architectures generally. This is attributed to the number of classes of streets where there are 11 classes in San Francisco and 10 classes in Boston, the context of \textit{Downtown Residential} is absent for the city of Boston as discussed earlier.
\begin{center}
\begin{table}[ht!]
    \centering
    	\caption{The accuracy of CNN architectures on validation dataset for Boston and San Francisco.}
	\begin{tabular}{|l|c|c|}
		\hline
		CNN/city             & Boston & San Francisco   \\ \hline
		ResNet18                  &  85.64\%    &  81.72\%                 \\ \hline
		ResNet34  &   85.45\%     &            82.02\%     \\ \hline
		ResNet50  &  85.64\%     &               82.71\%  \\ \hline
		AlexNet    &  83.16\%     &         81.69\%    \\ \hline
		Inception-v3	 &  87.79\% &               84.17\%  \\ \hline
	\end{tabular}
 \label{tab:accuraciesTable}
\end{table}
\end{center}

\begin{figure*}[!h]
	\advance\leftskip-4cm
	\begin{center}
		\includegraphics[width=0.8\linewidth]{plots/confusionMatrices.pdf}
		\caption{ The confusion matrix for the Inception-v3 model trained on Boston and San Francisco from left to right. The vertical axis has the true labels and the horizontal axis has the predicted labels by the model.}
		\label{fig:cmatresnet}
	\end{center}
\end{figure*}
\subsection{Visualizing the embedding space of street contexts}
Figure \ref{fig:tsne} visualizes the t-SNE projection of the feature vectors for each image in a sample from the training dataset. The feature vectors are the output values on the before last layer on the neural network (in our case we used the AlexNet model architecture). The feature vectors are 4096 dimensional. The t-SNE method help in visualizing the feature vector space by projecting it into a lower dimensional space while preserving neighborhood structure in the original space of the feature vectors\cite{maaten2008visualizing}. Figure \ref{fig:tsne} show the projection of feature vectors for a sample set of street images in Boston onto two dimensions.
 \begin{figure*}[!h]
	\advance\leftskip-4cm
	\begin{center}
		\includegraphics[width=158mm]{plots/tsne_cleaned-min.pdf}
		\caption{t-SNE visualization of the feature vectors on the 2d space for sample of images from the city of Boston}
		\label{fig:tsne}
	\end{center}
\end{figure*}
The t-SNE visualization shows the neighborhood structure of the highly dimensional spaces of feature vectors. The visualization illustrates the neighboring structure of the high dimensional space on the 2d in our case. The visualization shows the variations in streets in their contexts and geometrical features. Alleys present on the top right side of the plot are narrow and surrounded by red bricked building walls. Street passing through parks contexts are in the lower side of the plot with dense presence of greenery in them. Streets of type Downtown Commercial and Neighborhood Commercial share similar visual attributes to those of Alleys where they are usually surrounded by more buildings that have commercial signs, the Neighborhood Commercial sometimes has more vegetation. They reside on the top right side of the plot showing more of red-bricked buildings on the sides of the streets and little to no vegetation. Neighborhood Residential and Residential Throughway streets are more similar to Parks and have significant presence of greenery in Boston, they reside in the lower right to middle side of the plot. Streets that are highways, highway ramps and industrial contexts reside on the left side of the plot. They are usually wide and have less greenery or presence of buildings on the sides. Commercial Throughways are present closer to middle of the t-SNE visualization where they have some presence of greenery as well as businesses on the sides making them sit between Downtown-like streets streets and Park-like streets.
Figure \ref{fig:cmatresnet} shows the confusion matrices for the Inception-v3 model. The accuracy of the model typically varies by street context. In Boston, Inception-v3 has the highest accuracy for the Park context and lowest for Neighborhood Commercial context. We also notice a few cells where the model confuses streets contexts. For example, the model confuses Highways with Highway Ramps which share similar visual features. The model confuses Residential Throughways, Parks and Neighborhood Residential. They share the visual features of dense greenery on street sides. The model also confuses the Highways and Highway Ramps contexts. Generally, we notice that the cofusion patterns of the model are consistent with our t-SNE visualization where confused classes are usually in close proximity in the embedding space.  

For San Francisco, the model has the highest accuracy for the Alleys and lowest accuracy for classifying the Residential Throughways. The model confuses Downtown Commercial and Downtown Residential. Similar to Boston, the model confuses Highways and Highway Ramps. The mentioned confused classes share similar visual characteristics.

The patterns of confusion between classes in the city of Boston and San Francisco are similar. This is clear in the bottom right corner for the classes of Residential Throughway, Park and Neighborhood Residential. The same holds for Highways and Highway Ramps. In addition to Neighborhood Commercial and Neighborhood Residential. 

\subsection{Class Activation Mapping of street contexts}
To better understand the features which the model is looking for to classify streets. We further investigate the features attributing to the activations on the images using ideas of Class Activation Mapping (CAM) proposed by Zhou et al.\cite{zhou2016learning}. The methodology constructs a heat maps indicative of the features in images that are responsible for activating the predicted class. The heat map is generated by a weighted sum of the last set of convolutional outputs. The weights are of the last layer and corresponding to the outputted class node on the network.

%\textbf{Saliency maps for the predictions of the model}
%It would be great if we could get the saliency maps for the model to figure out what visual features activates the model. Using this we can futher invistigate the confusions of the model to understand why the model is confusing certain classes.

\begin{figure*}[!t]
	\advance\leftskip-4cm
	\begin{center}
		\includegraphics[width=\linewidth]{plots/CAM-min.pdf}
		\caption{Class activation mapping for street contexts classification in Boston using ResNet18}
		\label{fig:CAM}
	\end{center}
\end{figure*}
Figure \ref{fig:CAM} shows CAM applied to the ResNet18 model for the city of Boston. We show here a sample of the heat maps illustrating some of the features in the street view images that activated certain classification. The model captures several features in images and we discuss some of those shown in Figure \ref{fig:CAM}. For the Alleys class in the figure, the heat map of the CAM highlights red bricked walls, trash bins and back-side parking spots which are features typical for Alleys in the city of Boston. 


For Commercial Throughways, we see the activation map highlighting stores on the side of streets, the sidewalk and traffic lights. For Downtown Commercial, we see the activation map hot on high rise buildings typically available in downtown areas. For the Industrial streets, we see the model activated by corrugated steel walls and a cargo truck. For Neighborhood Residential, we see the model was activated by the presence of houses on the side of the street as well as greenery and cars parked on the side. For Neighborhood Commercial, we see the model activated by buildings with stores in them, we also notice the zebra line on the street under the heated activation area. For Parks, the model is activated by trees on the sides of the street. For Residential Throughways, the heated area is often wide to capture the throughway nature of the streets as well as detecting residential houses on the sides. For Highways, the heatmaps highlights the road area of the image on both lanes if exists.  For Highway Ramps, the model is looking at the road ahead which has less number of lanes usually. It is also slightly activated by the presence of a nighboring highway or bridge on which it will merge. These are sample activation features among others that the ResNet18 model highlights towards activating their respective predicted classes. In the Figure \ref{fig:CAM} we show a sample of two images per class for illustration and validation. %We include further CAM samples on the project page on \texttt{github}\footnote{https://github.com/fha/streetContext}.




==> intro.tex <==
\section{Introduction}
%\begin{itemize}
%\item here goes the motivation of the problem. Answer the following question:
%\item what is the problem, where does it come from?
%\item why is this problem important, namely why do we need street context classification? 
%\item where can this be used and for what purposes?
%\item its possible to link the work to self driving cars. one way is to say that self driving cars can benefit from knowing the context of streets? They should be more cautious to pedestrians when traveling in commercial areas and parks.
%\end{itemize}

%Cities today are growing very rapidly and are expected to be home for around 70 percent of world's population by 2050\cite{rode2011cities}. With the rapid urban population growth, cities' infrastructures are becoming data generation engines while needing to coop with the rapid growth in population. To coop with rapid growth of cities, urban planners are continuously innovating and revisiting methods and techniques of planning and design. With the rapid ubiquity of the internet and communication technologies, the internet is increasingly becoming home to large datasets pertaining to cities. In this paper, we explore one way to take advantage of the availability of city street view imagery to help city authorities and planners with street classification faster and at larger scales in an automatic fashion.

%the existing classification methods and the SF prpoposed method
Cities today are growing very rapidly and are expected to be home for around 70 percent of world's population by 2050\cite{rode2011cities}. Transportation engineers and urban planners traditionally classified streets on the road network in cities based on vehicular transportational features. Such street classifications include arterials, major roads, minor roads, connectors and so forth. Although such classification is very useful in terms of vehicular transportation planning, it doesn't differentiate between streets that pass through residential versus commercial areas for example, where the differentiation is of at most importance to design and build more livable and sustainable streets. Recently, a significant emphasis to increase focus on the \textit{context} of a street in the process of urban planning have become very noticeable. The \textit{context} of a street encompasses the use of land on the sides of a street in addition to its vehicular transportational characteristics. 

Several city and state authorities have started proposing extensions for the traditional classification of roads towards one that encompass the use of the sides of the streets.  For example, chapter 4 of the guidebook for transportation planning from the state of Pennselvania elaborates on the supremacy of \textit{street context} over traditional transportation classification methods for purposes of developing more livable and sustainable cities\cite{guidebook2008planning}.  The state of Florida Department of Transportation (FDOT) started adopting new classification methods of \textit{street context} that goes beyond the traditional classifications of streets\cite{FDOT_ContextClassification}.  The city of San Francisco adopted an extended street classification scheme to govern how the city designs, builds, and maintains its pedestrian environment, the classification scheme is called the Better Street Plan (BSP). The intent for it is to become the corner stone for developing streets that are more livable\cite{SF_BSP}. In this paper, we illustrate a way to automate the process of BSP classification of streets in San Francisco and Boston using computer vision and street view imagery. 

%Computer vision is one of the prominent areas of machine learning and AI, it employs approaches and techniques from machine learning for computers to develop models with high level understanding of images and videos data. The recent developments in the area of deep learning have been very successful in tasks such as image classification, object recognition and detection. The scientific domain of applications hasn't been of a particular focus for researchers developing the method most of the time. This provides room for researchers to contribute in applying computer vision to application domains. 

%The following section starts with an exploration of the potentials of using deep learning with street view images to develop a tool that can aid in the process of city planning.

 978-1-7281-0858-2/19/$31.00 © 2019 IEEE 
 
With the ubiquity of technology today, we have access to data on massive scales that can alleviate challenges of urban data collection and tedious data entry\cite{zheng2014urban}. There has been applications in domains of urban sciences, transportation and socio-economic sciences\cite{lazer2009life,alhasoun2017city,zhang2018social}. Its is also at the core of the relatively new field of urban computing\cite{zheng2014urban}. An example of data that became available with the ubiquity of technology in cities is street imagery data. The dataset is usually collected by moving cars with cameras. The data is then aggregated and used for the public to browse and view different places. Example efforts of such data collection include the Google Street View\cite{streetViewApi}. Another example of effort of crowd sourcing the collection of street view imagery includes Mapilary which proved successful at collecting considerably large amounts of street imagery data worldwide\cite{mapilary}. We aim to show that this dataset can be used with models of computer vision to aid urban development.

We summarize our contributions in the following points:
\begin{itemize}
\item We develop the framework for building automatic \textit{street context} classification. The framework is composed of labeling and sampling street view imagery. Then training and validation of deep convolutional neural network models.
\item We test the framework on data gathered from the wild. Namely the cities of San Francisco and Boston where we have labeled \textit{street contexts}.
\item We illustrate the potential of such applications by reporting on CNNs achieving accuracies in the 81\% to 87\% range. 

\item  We then validate our models using t-SNE to visualize the streets embedding space. We apply Class Activation Mapping (CAM) methods for interpretability of the predicted classes\footnote{https://github.com/fha/streetContext}.
\end{itemize}





